Point-of-Interest Recommendation: Exploiting Self-Attentive Autoencoders with Neighbor-Aware Influence

The rapid growth of Location-based Social Networks (LBSNs) provides a great opportunity to satisfy the strong demand for personalized Point-of-Interest (POI) recommendation services. However, with the tremendous increase of users and POIs, POI recommender systems still face several challenging problems: (1) the hardness of modeling non-linear user-POI interactions from implicit feedback; (2) the difficulty of incorporating context information such as POIs' geographical coordinates. To cope with these challenges, we propose a novel autoencoder-based model to learn the non-linear user-POI relations, namely \textit{SAE-NAD}, which consists of a self-attentive encoder (SAE) and a neighbor-aware decoder (NAD). In particular, unlike previous works equally treat users' checked-in POIs, our self-attentive encoder adaptively differentiates the user preference degrees in multiple aspects, by adopting a multi-dimensional attention mechanism. To incorporate the geographical context information, we propose a neighbor-aware decoder to make users' reachability higher on the similar and nearby neighbors of checked-in POIs, which is achieved by the inner product of POI embeddings together with the radial basis function (RBF) kernel. To evaluate the proposed model, we conduct extensive experiments on three real-world datasets with many state-of-the-art baseline methods and evaluation metrics. The experimental results demonstrate the effectiveness of our model.

==> backup/methods0512.tex <==

\section{Preliminaries}
In this section, we first introduce the definitions and notations. Then we review the basic ideas of autoencoders.

\subsection{Definition and Notation}
For ease of illustration, we first summarize the definitions and notations.

\textit{Definition 1}. (\textbf{POI}) A POI is defined as a uniquely identified site (e.g., a restaurant) with two attributes: an identifier and geographical coordinates (latitude and longitude).

\textit{Definition 2}. (\textbf{Check-in}) A check-in is a record that demonstrates a user has visited a POI at a certain time. A user's check-in is represented by a 3-tuple: user ID, POI ID and the timestamp.

\textit{Definition 3}. (\textbf{POI Recommendation}) Given users' check-in records, POI recommendation aims at recommending a list of POIs for each user that the user is interested in but never visited.

\begin{table}[h]
\centering
\caption{List of notations.}
\label{tab:notations}
\begin{tabular}{ll}
 \hline
$ M $, $ N $ & the number of users and POIs \\
$ \mathbf{X} $, $ \hat{\mathbf{X}} $ & the input data and reconstructed data \\
$ \mathbf{R} $ & the check-in frequency matrix \\
$ \mathbf{C} $ & the confidence matrix \\
$ \mathbf{W}_{*} $, $ \mathbf{b}_{*} $ & the weight matrix and bias vector \\
$ a_{*} $ & the activation function \\
$ D $, $ \eta $ & the parameters of the weighting scheme \\
$ H $ & the hidden dimension \\
$ \beta $, $ \lambda $ & the regularization terms \\ \hline
\end{tabular}
\end{table}


POI recommendation is commonly studied on a user-POI matrix $ \mathbf{R} \in \mathbb{N}^{M \times N} $, where there are $ M $ users and $ N $ locations, each entry $ r_{u,i} $ represents the frequency user $ u $ checked-in at location $ i $. We denote the binary rating matrix as $ \mathbf{X} \in \mathbb{N}^{M \times N} $, where each entry $ x_{u,i} \in \{0,1\} $ indicates whether user $ u $ has visited location $ i $. The terms POI and location are used interchangeably in this paper. Here, following common symbolic notation, upper case bold letters denote matrices, lower case bold letters denote column vectors without any specification, and non-bold letters represent scalars. The notations are shown in Table \ref{tab:notations}.

\subsection{Autoencoders} \label{subsec:autoencoder}
A single hidden-layer autoencoder (AE) is an unsupervised neural network, which is composed of two parts, i.e., the encoder and decoder. The encoder has one activation function that maps the input data to the latent space. The decoder also has one activation function mapping the representations in the latent space to the reconstruction space. Given the input $ \mathbf{x}_{i} $, a single hidden-layer autoencoder is shown as follows:
\begin{equation}
\begin{aligned}
& encoder: \mathbf{z}_{i} = a_{1}(\mathbf{W}_{1} \mathbf{x}_{i} + \mathbf{b}_{1}) \\
& decoder: \hat{\mathbf{x}}_{i} = a_{2}(\mathbf{W}_{2} \mathbf{z}_{i} + \mathbf{b}_{2}),
\end{aligned}
\label{eq:encoder_and_decoder}
\end{equation}
where $ \mathbf{W}_{*} (\mathbf{W}_{1} \in \mathbb{R}^{H \times N}), \mathbf{W}_{2} \in \mathbb{R}^{N \times H}) $, $ \mathbf{b}_{*} $ and $ a_{*} $ denote the weight matrix, bias vector and activation function, respectively. $ \hat{\mathbf{x}}_{i} $ is the reconstructed version of $ \mathbf{x}_{i} $. The output of the encoder $ \mathbf{z}_{i} $ is the representation of $ \mathbf{x}_{i} $ in the latent space. The goal of the autoencoder is to minimize the reconstruction error of the output and the input. The loss function is shown as follows:
\begin{equation}
\mathcal{L}_{AE} = \sum_{i = 1}^{M}||\mathbf{x}_{i} - \hat{\mathbf{x}}_{i}||_{2}^{2}.
\label{eq:autoencoder_loss_function}
\end{equation}

\textbf{Relations to Matrix Factorization}. One reason that the autoencoder is capable of recommendation is that its formulation is much similar to the classical matrix factorization \cite{DBLP:journals/computer/KorenBV09}. Let we denote $ \mathbf{U} $ and $ \mathbf{V} $ as user latent factors and item latent factors, respectively, where $ \mathbf{V} $ has the same dimension with $ \mathbf{W}_{2}. $ If $ a_{2} $ is set to the identity function, then the formula in Eq. \ref{eq:encoder_and_decoder} can be rephrased as follows:
\begin{equation}
\begin{aligned}
 & \mathbf{u}_{i} = a_{1}(\mathbf{W}_{1} \mathbf{x}_{i} + \mathbf{b}_{1}) \\
 & \hat{\mathbf{r}}_{i} = \mathbf{V} \mathbf{u}_{i} + \mathbf{b}_{2} \Rightarrow \hat{r}_{i,j} = \mathbf{u}_{i}^{\top} \mathbf{v}_{j} + b_{2}^{(j)} 
\end{aligned}
\label{eq:relation_to_MF}
\end{equation}
where $ \hat{r}_{i,j} $ is the predicted rating of a user $ i $ on a POI $ j $, $ b_{2}^{(j)} $ is the $ j $-th element of $ \mathbf{b}_{2} $, which can be treated as the item bias. The rephrased formula demonstrates the strong similarity between autoencoders and matrix factorization in recommendation, which makes autoencoders have the ability to recommend items.

\textbf{Relations to word2vec}. word2vec \cite{DBLP:conf/nips/MikolovSCCD13} is an effective and scalable method to learn embedding representations in word sequences, modeling words' contextual correlations in word sentences. word2vec utilizes either of two model architectures to produce a distributed representation of words: continuous bag-of-words (CBOW) or continuous skip-gram. Take continuous skip-gram for example, the input of the model is an one-hot vector to represent the current word, then the model uses the current word to predict the surrounding window of context words. This model is highly similar to AE when the input of AE is an one-hot vector. If the current word is $ i $ and target word is $ j $, we set the activation function to identity and bias to zero, then the output of the decoder is:
\begin{equation}
\hat{x}_{ij} = \mathbf{W}_{2}^{(j) \top} \mathbf{W}_{1}^{(i)},
\end{equation}
where $ \mathbf{W}_{1}^{(i)} $ and $ \mathbf{W}_{2}^{(j)} $ are the rows of $ \mathbf{W}_{1} $ and $ \mathbf{W}_{2} $, respectively. If we further apply Softmax on the output of the decoder:
\begin{equation}
P(l_{j}|l_{i}) = \frac{exp(\hat{x}_{ij})}{\sum_{j=1}^{N} exp(\hat{x}_{ij})},
\end{equation}
where this probability shows how likely the word $ j $ will appear in the window of the current word $ i $. In our POI recommendation setting, this formula demonstrates if a user has checked-in location $ l_{i} $, how likely the user would check-in location $ l_{j} $. Therefore, the product of $ \mathbf{W}_{1}^{(i)} $ and $ \mathbf{W}_{2}^{(j)} $ can be used for capturing the relation between $ l_{i} $ and $ l_{j} $.

\section{Methodologies}
In this section, we introduce the proposed model for POI recommendation, which consists of two components, i.e., a self-attentive encoder and a neighbor-aware decoder, demonstrating in Figure \ref{fig:model_architecture}. We first present the stacked autoencoder as our major building block. Then we illustrate the self-attentive encoder to adaptively select representative POIs that can reflect users' preferences. Next, we demonstrate the neighbor-aware decoder to model the geographical influence in POI recommendation, which is a phenomenon that users tend to check-in those unvisited POIs that close to a POI that they checked-in before. Lastly we present the loss function for implicit feedback and how to optimize the model based on the loss function.

\subsection{Model Basics} \label{subsec:model_basics}
To learn the user hidden representation and reconstruct user preferences on unvisited POIs, we propose to adopt a stacked autoencoder, where the deep network architecture and non-linear activations can capture the non-linear and complex user-POI interactions \cite{DBLP:conf/www/HeLZNHC17}. Formally, the stacked autoencoder is shown as follows:
\begin{equation}
enc:
\begin{cases}
\mathbf{z}_{u}^{(1)} = a_{1}(\mathbf{W}_{1} \mathbf{x}_{u} + \mathbf{b}_{1}) \\
\mathbf{z}_{u} = a_{2}(\mathbf{W}_{2} \mathbf{z}_{u}^{(1)} + \mathbf{b}_{2})
\end{cases}
dec:
\begin{cases}
\mathbf{z}_{u}^{(3)} = a_{3}(\mathbf{W}_{3} \mathbf{z}_{u} + \mathbf{b}_{3}) \\
\hat{\mathbf{x}}_{u} = a_{4}(\mathbf{W}_{4} \mathbf{z}_{u}^{(3)} + \mathbf{b}_{4})
\end{cases}
\label{eq:deep_AE}
\end{equation}
where $ \mathbf{W}_{1} \in \mathbb{R}^{H_{1} \times N} $, $ \mathbf{W}_{2} \in \mathbb{R}^{H \times H_{1}} $, $ \mathbf{W}_{3} \in \mathbb{R}^{H_{1} \times H} $ and $ \mathbf{W}_{4} \in \mathbb{R}^{N \times H_{1}} $ are parameter matrices of the stacked AE. $ H_{1} $ is the dimension of the first hidden layer, and $ H $ is the dimension of the bottleneck layer. $ \mathbf{z}_{u} $ and $ \hat{\mathbf{x}}_{u} $ are the hidden representation and reconstructed ratings of user $ u $, respectively.

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{pic/whole.pdf}
        \caption{\label{fig:whole_model}Whole Model}
    \end{subfigure}%
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{pic/encoder.pdf}
        \caption{\label{fig:encoder}Encoder}
    \end{subfigure}%
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{pic/decoder.pdf}
        \caption{\label{fig:decoder}Decoder}
    \end{subfigure}
    \caption{\label{fig:model_architecture}The model architecture.}
\vspace{-0.3cm}
\end{figure*}


\subsection{Self-Attentive Encoder} \label{subsec:self-attention}
As we presented in section \ref{subsec:model_basics}, we apply a stacked AE to learn users' hidden representations. In the proposed model, the input is a multi-hot user vector $ \mathbf{x}_{i} \in \mathbb{R}^{N} $, where 1 indicates the user has been to a certain POI. As we discussed in section \ref{subsec:autoencoder}, autoencoder is largely similar to the word2vec model under certain circumstance. Inspired by the word2vec model, we can also treat $ \mathbf{W}_{1} $ in autoencoder as the embedding of all POIs. Thus, the encoder part works as follows: (1) given a user's check-in set $ L_{u} = \{l_{1},...,l_{n}\} $, corresponding POIs' embeddings in $ \mathbf{W}_{1} $ are selected and summed; (2) after having the summed embedding, perform the activation function to get the user hidden representation. Here, the summed embedding acts as a context vector for the decoder. Then the decoder predicts under this context which POI will be visited.

Since the model input are multi-hot vectors, which makes each embedding in $ \mathbf{W}_{1}[L_{u}] $ equally contribute to the user hidden representation, where $ [\cdot] $ is the slicing operation that selects corresponding vectors to form a sub-matrix of $ \mathbf{W}_{1} $, which has the size $ H_{1} $-by-$ n $:
\begin{equation}
\mathbf{W}_{1}[L_{u}] = (\mathbf{W}_{1}^{(l_{1})}, \mathbf{W}_{1}^{(l_{2})},..., \mathbf{W}_{1}^{(l_{n})})
\label{eq:slice_operation}
\end{equation}
However, in the user check-in history, there should be some POIs more representative than others that can directly reflect user's preference. Thus, these representative POIs should contribute more to user hidden representations. This intuition inspires us to propose a self-attentive mechanism, which learns a weighted sum of embeddings in $ \mathbf{W}_{1}[L_{u}] $ to form the user latent representation.

The goal of the self-attention model is to select POIs that are representative to users' preferences and then weighted aggregate all the embeddings of all checked-in POIs to characterize users. Given checked-in POI embeddings of a user $ \mathbf{W}_{1}[L_{u}] $, we use a two-layer network without bias to compute the attention score:
\begin{equation}
\mathbf{a}_{u} = softmax(tanh(\mathbf{w}_{a}^{\top} \mathbf{W}_{1}[L_{u}]))
\label{eq:attention_vector}
\end{equation}
where $ \mathbf{w}_{a} \in \mathbb{R}^{H_{1}} $ is the transformation attention vector to be learned. Then we sum up the embeddings in $ \mathbf{W}_{1}[L_{u}] $ according to the weight provided by $ \mathbf{a}_{u} $ to get a vector representation of the user:
\begin{equation}
\mathbf{z}_{u}^{(1)} = \sum_{l_j \in L_u} a_{u,j} \mathbf{W}_1[l_j]
\end{equation}

However, experimental results show that the standard attention solution works poorly in our scenario. The major reason is that the size of different user check-in sets varies a lot, while in conventional applications of attention such as NLP tasks, the number of attentive components does not vary much, such as words in sentences. Moreover, by applying \ref{eq:attention_vector}, the $ softmax $ function performs $ L1 $ normalization on attention weights, which may overly punish the weights and make one or two weights dominate the whole attention vector. 

To tackle the above problem, we adopt a matrix to capture the multiple-hop attention \cite{DBLP:journals/corr/LinFSYXZB17}. Each hop of the attention represents an aspect of relations among all embeddings in $ \mathbf{W}_{1}[L_{u}] $. Suppose we want $ d_{a} $ aspects of attention to be extracted from the embeddings, then we can extend $ \mathbf{w}_{a} $ to $ \mathbf{W}_{a} \in \mathbb{R}^{d_{a} \times H_{1} } $:
\begin{equation}
\mathbf{A}_{u} = softmax(tanh(\mathbf{W}_{a} \mathbf{W}_{1}[L_{u}]),dim=1)
\label{eq:attention_matrix}
\end{equation}
where $ \mathbf{A}_{u} \in \mathbb{R}^{d_{a} \times n} $ is the attention matrix, the $ softmax $ is performed along the second dimension of its input. By multiplying the attention matrix and the item embeddings, we have the matrix representation of a user $ u $:
\begin{equation}
\mathbf{Z}_{u}^{(1)} = \mathbf{A}_{u} \mathbf{W}_{1}^{\top}[L_{u}]
\label{eq:user_embedding_matrix}
\end{equation}
where $ \mathbf{Z}_{u} \in \mathbb{R}^{d_{a} \times H_{1}} $ is the matrix representation of the user $ u $, which is not suitable for our decoder. Thus, we have one more neural layer to aggregate attention from different aspects into one aspect. Then the hidden representation of user $ u $ is revised as:
\begin{equation}
\mathbf{z}_{u}^{(1)} = a_{t}(\mathbf{Z}_{u}^{(1) \top} \mathbf{w}_{t} + \mathbf{b}_{t})
\label{eq:user_embedding}
\end{equation}
where $ \mathbf{w}_{t} \in \mathbb{R}^{d_{a}} $ is transition vector in the aggregation layer.

\subsection{Neighbor-Aware Decoder} \label{subsec:neighbor_influence}
In LBSNs, there are physical distances between users and POIs, which is a unique property distinguishing POI recommendation from other recommendation tasks. In POI recommendation, a user's occurrences are typically constrained in several certain areas. This is the well-known geographical clustering phenomenon (a.k.a geographical influence) in users' check-in activities, has been exploited to largely improve the POI recommendation performance. Different from most of the previous studies that mainly exploit geographical influence from a user's perspective (learning the geographical distribution of each individual user's check-ins), the proposed neighbor-aware influence model captures the geographical influence from a POI's perspective. 

According to aforementioned geographical influence, one intuition contributes to this phenomenon: users prefer to visit nearby POIs and check-in POIs surrounded a POI that they visited before. From this intuition, a checked-in POI may have impacts on other unvisited POIs. And the impact level is determined by the properties and distance of two POIs. Inspired by the word2vec, which applies inner product to model the relation between a source word and a target word, we also leverage similar techniques to model the influence a checked-in POI exerts on unvisited POIs (section \ref{subsec:autoencoder}, relations to word2vec).

Formally, given a user's check-in set $ L_{u} = \{l_{1},...,l_{n}\} $, the influence checked-in POIs exerted on unvisited POIs is shown:
\begin{equation}
\mathbf{P}_{u} = \mathbf{W}_{4} \cdot \mathbf{W}_{1}[L_{u}],
\end{equation}
where $ \mathbf{P}_{u} \in \mathbb{R}^{N \times n} $. Each column of $ \mathbf{P}_{u} $ is the correlation between a certain checked-in POI and all other POIs (the correlation on itself is set to 0).

The above inner product method gives a basic indication about how related two POIs are, however, it does not explicitly take the distance between two POIs into consideration. According to Tobler's First Law of Geography--everything is related to everything else, but near things are more related than distant things. To further make two nearby POIs correlated, we adopt the Gaussian radial basis function kernel (RBF kernel) to model the relation between two POIs from the perspective of geographical distance:
\begin{equation}
K(l_{i},l_{j}) = exp(-\gamma ||\mathbf{l}_{i} - \mathbf{l}_{j}||^{2}),
\label{eq:rbf_kernel}
\end{equation}
where $ \mathbf{l}_{i} $ and $ \mathbf{l}_{j} $ are the geographical coordinates of POIs. $ \gamma > 0 $ is a hyperparameter to control the geographical correlation level of two given POIs. The value range of RBF kernel is $ K(l_{i},l_{j}) \in [0, 1] $, for computation simplicity, if the value of $ K(l_{i},l_{j}) $ is less than 0.1, we set it to 0.
% This setting makes the influence radius of a checked-in POI to be 15km. 

By incorporating the RBF kernel, our neighbor-aware influence model is shown:
\begin{equation}
\mathbf{P}_{u} = (\mathbf{W}_{4} \cdot \mathbf{W}_{1}[L_{u}]) \odot \mathbf{K}[L_{u}],
\label{eq:neighbor_influence_matrix}
\end{equation}
where $ \mathbf{K}[L_{u}] \in \mathbb{R}^{N \times n} $ is the RBF kernel value from Eq. \ref{eq:rbf_kernel}, $ \odot $ is the element-wise multiplication. 

To obtain the accumulated influence from all checked-in POIs, we sum along the row of $ \mathbf{P}_{u} $ to get $ \mathbf{p}_{u} \in \mathbb{R}^{N} $:
\begin{equation}
\mathbf{p}_{u} = \sum_{j=1}^{n} \mathbf{P}_{u} ^ {(i,j)}, i=1,2,...,N
\label{eq:neighbor_influence_vector}
\end{equation}
Then the decoder of the proposed model can be represented as:
\begin{equation}
\hat{\mathbf{x}}_{u} = a_{4}(\mathbf{W}_{4} \mathbf{z}_{u}^{(3)} + \mathbf{b}_{4} + \mathbf{p}_{u})
\label{eq:neighbor_aware_decoder}
\end{equation}

\textbf{Relations to word2vec}.

\textbf{Relations to attention mechanism in machine translation}.


\subsection{Weighted Loss for Implicit Feedback} \label{subsec:weighted_AE}
Generally, there are two kinds of data used to capture user preferences in recommendation tasks, i.e., explicit feedback and implicit feedback. Explicit feedback directly reflects how much a user prefers an item, such as star ratings on Netflix. In such cases, users not only reveal their favorite movies with high ratings, but also their least favorite movies with low ratings. 

In POI recommendation, check-in data is treated as implicit feedback. Since a user's check-in records only include the locations she visited, and the visit frequency indicates the confidence level of her preference. Therefore, there are only \textit{positive} examples observed in the check-in records, which makes POI recommendation an One Class Collaborative Filtering (OCCF) problem \cite{DBLP:conf/icdm/PanZCLLSY08,DBLP:conf/icdm/HuKV08}. 

To tackle the OCCF problem and capture user preferences from check-in data, we adopt a general weighting scheme to distinguish visited and unvisited POIs. Specifically, we consider all unvisited locations as negative examples, and assign the weights of all negative examples to a same value, e.g., 1. As for visited locations, the weights are increased monotonically with users' check-in frequencies. With such a weighting scheme, our model not only distinguishes visited and unvisited POIs, but also discriminates the preference degrees of all visited POIs. The objective function for implicit feedback is presented as follows,
\begin{equation}
\mathcal{L}_{WAE} = \sum_{u = 1}^{M} \sum_{i=1}^{N}||c_{u,i} (x_{u,i} - \hat{x}_{u,i})||_{2}^{2} = ||\mathbf{C} \odot (\mathbf{X}-\mathbf{\hat{X}})||^{2}_{F},
\label{eq:weighted_autoencoder_loss_function}
\end{equation}
where $ \odot $ is the element-wise multiplication of matrices. $ ||\cdot||_{F} $ is the Frobenius norm of matrices. In particular, we set the confidence matrix $ \mathbf{C} \in \mathbb{R}^{M \times N} $ as follows, 
\begin{equation}
c_{u,i}=
\begin{cases}
\varphi(r_{u,i}) + 1 & \text{ if } r_{u,i} > 0 \\ 
1 & \text{} otherwise
\end{cases}
\label{eq:weight_function}
\end{equation}
where $ \gamma(r_{u,i}) > 0 $ is a monotonically increasing function with respect to $ r_{u,i} $. This setting exactly encodes the observation that the frequency is a confidence of user preferences. This weighted autoencoder is a general model and can be used in other recommendation tasks that take implicit feedback as input.

\subsection{Network Training}
By combining regularization terms, the objective function of the proposed model is shown as follows:
\begin{equation}
\begin{aligned}
\mathcal{L} =||\mathbf{C} \odot (\mathbf{X}-\mathbf{\hat{X}})||^{2}_{F} + \lambda(||\mathbf{W}_{*}||^{2}_{F} + ||\mathbf{w}_{t}||^{2}_{2}),
\end{aligned}
\label{eq:final_loss}
\end{equation}
where $ \lambda $ is the regularization parameter, $ \mathbf{W}_{*} $ includes $ \mathbf{W}_{1} $, $ \mathbf{W}_{2} $, $ \mathbf{W}_{3} $, $ \mathbf{W}_{4} $ and $ \mathbf{W}_{a} $. By minimizing the objective function, the partial derivatives with respect to all the parameters can be computed by gradient descent with back-propagation. And we apply Adam \cite{DBLP:journals/corr/KingmaB14} to automatically adapt the learning rate during the learning procedure. The mini-batch training algorithm is presented in Alg. \ref{alg:batch_training_algorithm}. 

\begin{algorithm}
  \textbf{Input}: $ \mathbf{X} $, $ \mathbf{C} $, $ I $ \;
  % \KwIn{$ \mathbf{X} $, $ \mathbf{C} $, $ I $}
  % \KwOut{the reconstructed matrix $ \hat{\mathbf{X}} $}
  Initialize parameters $ \mathbf{W}_{*} $, $ \mathbf{w}_{t} $, $ \mathbf{b}_{*} $ \;
  numBatches = $ M $ $/$ $ batchSize $ \;
  \While{iter < I} {
    Shuffle($ \mathbf{X}, \mathbf{C} $) \;
    \For{batchID = 0; batchID < numBatches; batchID++} {
      $ \mathbf{X}_{batch}, \mathbf{C}_{batch} $ = ExtractBatchData(batchID, $ \mathbf{X}, \mathbf{C} $) \;
      For each user $ u $ in $ \mathbf{X}_{batch} $, apply Eq. \ref{eq:slice_operation} to get $ \mathbf{W}_{1}[L_{u}] $ \;
      Apply Eq. \ref{eq:attention_matrix}, Eq. \ref{eq:user_embedding_matrix} and Eq. \ref{eq:user_embedding} to get $ \mathbf{z}_{u}^{(1)} $ \;
      Apply Eq. \ref{eq:neighbor_influence_matrix} and Eq. \ref{eq:neighbor_influence_vector} to get $ \mathbf{p}_{u} $ \;
      Concatenate each $ \mathbf{z}_{u}^{(1)} $ and $ \mathbf{p}_{u} $ in the batch, respectively \;
      Apply Eq. \ref{eq:deep_AE} and \ref{eq:neighbor_aware_decoder} to get $ \hat{\mathbf{X}}_{batch} $ \;
      Apply Eq. \ref{eq:final_loss} to obtain $ \mathcal{L}_{batch} $ and back-propagate the error through the entire network \;
    }
  }
  % \Return{$ \hat{\mathbf{X}} $}

\caption{Training Algorithm}
\label{alg:batch_training_algorithm}
\end{algorithm}

\textbf{Recommendation}. At prediction time, the proposed model takes each user's binary rating vector $ \mathbf{x}_{i} $ as input and obtains the reconstructed rating vector $ \hat{\mathbf{x}}_{i} $ as output. Then the POIs that are not in training set and have largest prediction scores in $ \hat{\mathbf{x}}_{i} $ are recommended to the user.




==> preliminaries.tex <==


\section{Methods}
In this section, we demonstrate the proposed methodology for the task of POI recommendations, which takes POI similarities, user preferences and geographical influence into account.


\subsection{Notation}
Suppose there are $ N $ users and $ M $ locations. We denote the set of all locations as $ L $. For convenience we will henceforth refer to $ u $ as user and $ l $ as location. The terms location and POI are used interchangeably in this paper. In addition, the sequence a user $ u $ checked-in is denoted as $  S_{u} $, and the set a user $ u $ checked-in is referred to $  L_{u} $. Following common symbolic notation, upper case bold letters denote matrices, lower case bold letters denote column vectors without any specification, and non-bold letters represent scalars.







